Electromagnetic processes in a $\chi$EFT framework

Recently, we have derived a two--nucleon potential and consistent nuclear electromagnetic currents in chiral effective field theory with pions and nucleons as explicit degrees of freedom. The calculation of the currents has been carried out to include N$^3$LO corrections, consisting of two--pion exchange and contact contributions. The latter involve unknown low-energy constants (LECs), some of which have been fixed by fitting the $np$ S- and P-wave phase shifts up to 100 MeV lab energies. The remaining LECs entering the current operator are determined so as to reproduce the experimental deuteron and trinucleon magnetic moments, as well as the $np$ cross section. This electromagnetic current operator is utilized to study the $nd$ and $n^3$He radiative captures at thermal neutron energies. Here we discuss our results stressing on the important role played by the LECs in reproducing the experimental data.

==> cpc-hepnp.tex <==
%%
%% This is file `cpc-hepnp.cls',
%% 
%% Copyright (c) 2007 Chinese Physics C
%% http://cpc-hepnp.ihep.ac.cn
%% mailto:hepnp@ihep.ac.cn

%------------------------------------------------------------------------------------------------------

\NeedsTeXFormat{LaTeX2e}[1996/12/01]
\ProvidesClass{cpc-hepnp}
\def\class@name{cpc-hepnp}%

\NeedsTeXFormat{LaTeX2e}
   \@obsoletefile{article.cls}{article.sty}
   \LoadClass{article}

\RequirePackage{fancyhdr}
\RequirePackage[numbers,sort&compress]{natbib}

\DeclareMathSizes{10}{10}{6}{5}  

%£?£?£?£?£?£?£?£?£?£?£?£?£?£?£?£?£?£?£?£?£?£?£?£?£?£?£?£?£?£?£?£?£?£?£?£?£?£?£?£?£?£?£?£?£?£?£?£?£?£?£?£?

\setlength{\textheight}{242mm}
\setlength{\textwidth}{169mm}
\setlength{\topmargin}{-0.3in}  
\leftmargin 0mm
\evensidemargin 0mm
\headheight 12mm               
\headsep 5mm                  
\footskip 11pt                   
\oddsidemargin-8mm             
\evensidemargin-8mm            
\columnsep 7mm               

%--------------------------------------------------------------------------------------------------------------

\renewcommand{\baselinestretch}{1.1}  
\renewcommand{\arraystretch}{1.2}

\setlength{\parskip}{0pt}       
\setlength{\floatsep}{6pt}         
\setlength{\textfloatsep}{6pt}    
\setlength\footnotesep{8pt}        

\setlength{\abovecaptionskip}{4pt plus1pt minus1pt}
\setlength{\belowcaptionskip}{4pt plus1pt minus1pt} 
\setlength{\abovedisplayskip}{6pt plus1pt minus1pt}
\setlength{\belowdisplayskip}{6pt plus1pt minus1pt} 
\addtolength{\thinmuskip}{-1mu}         
\addtolength{\medmuskip}{-2mu}      
\addtolength{\thickmuskip}{-2mu}      


%---------------------------------------------------------------------------------------------------

\font\scten=euex10 at 10pt
\newcommand{\vint}{\mathop{{\vcenter{\hbox{\scten\char90}}}}}
\renewcommand{\int}{\vint}

\font\sctenr=euex10 at 9pt
\newcommand{\sint}{\mathop{{\vcenter{\hbox{\sctenr\char82}}}}} 

\font\timeroman=psyr at 10pt
\newcommand{\vpartial}{\mathop{{\hbox{\timeroman \char182}}}} 


%---------------------------------------------------------------------------------------------------

\def\journal#1#2#3#4#5{{#1}. {#2}, {#3}, {\bf #4}: {#5}}
\def\book#1#2#3#4#5#6{{#1}. {#2}. {#3}: {#4}, {#5}. {#6}}
\def\diss#1#2#3#4#5#6#7{{#1}. {#2}. {#3}. {#4}: {#5}, {#6}. {#7}}

\newcommand{\thanksmark}{\textsuperscript{\,\rm{*}}}   


\newcommand{\ruleup}{\vspace*{-0.5cm}\noindent\rule{8.35cm}{0.2pt}\rule{0.6pt}{0.4cm}\vspace*{0.2cm}}
\newcommand{\ruledown}{\vspace*{-0.5cm}\hfill\noindent{\vspace*{-0.2cm}\lower.38cm\hbox{\rule{0.2pt}{0.4cm}}\rule{8.35cm}
              {0.2pt}}\vspace*{-3.5mm}}

\newcommand{\wen}[1]{\raisebox{0.3mm}{\textsuperscript{[#1]}}} 

\let\asas=\cite
\renewcommand\cite[1]{\raisebox{0.3mm}{\textsuperscript{\asas{#1}}}} 


\newcommand{\bb}{\raisebox{0.4mm}[0pt]{:}}


%----------------------------------\thanks, \footnote--------------------------------------

\makeatletter

\renewcommand{\thefootnote}{\fnsymbol{footnote}}  

\renewcommand{\thanks}[1]{\thanksmark
    \protected@xdef\@thanks{\@thanks
        \protect\footnotetext[0]{\hspace*{-6pt}$*$\;#1}}}

\newcounter{email}            
\setcounter{email}{1}
\newcommand{\email}[1]{%
    \protected@xdef\@thanks{\@thanks%
        \protect\footnotetext[0]{\hspace*{-8pt}\arabic{email})\,{E-mail:\,}#1}}%
        \stepcounter{email}}%



\renewcommand\footnoterule{%
  \kern 1\p@
  \hrule \@width37mm
  \kern 8\p@}

\renewcommand\@makefntext[1]{%
    \parindent 1em%
    \noindent
    \hb@xt@2em{\hss\@makefnmark}#1}

%---------------------------------------------------------------------------------------

\renewcommand\maketitle{\par%
  \begingroup
    \renewcommand\thefootnote{\@fnsymbol\c@footnote}%
    \def\@makefnmark{\rlap{\@textsuperscript{\normalfont\@thefnmark}}}%
    \long\def\@makefntext##1{\parindent 1em\noindent
            \hb@xt@2em{%
                \hss\@textsuperscript{\normalfont\@thefnmark}}##1}%
    \if@twocolumn
      \ifnum \col@number=\@ne
        \@maketitle
      \else
        \twocolumn[\@maketitle]%
      \fi
    \else
      \newpage
      \global\@topnum\z@   % Prevents figures from going at top of page.
      \@maketitle
    \fi
  \@thanks
  \endgroup
  \setcounter{footnote}{0}%
  \global\let\thanks\relax
  \global\let\maketitle\relax
  \global\let\@maketitle\relax
  \global\let\@thanks\@empty
  \global\let\@author\@empty
  \global\let\@date\@empty
  \global\let\@title\@empty
  \global\let\title\relax
  \global\let\author\relax
  \global\let\date\relax
  \global\let\and\relax}

\renewcommand\@maketitle{%
  \begin{center}%
  \let \footnote \thanks
   \vspace*{0.5em}
    {\LARGE\bf \@title \par}%
    {\normalsize%
      \lineskip .5em%
      \vskip 2em%
      \begin{tabular}[t]{c}%
        \@author%
      \end{tabular}}%
  \end{center}}%
\makeatother

%---------------------------------------------------------------------------------------------

\newcommand{\address}[1]{%
  \begin{center}%
    \vskip -1em%
    \begin{center}%
      {\footnotesize #1}%
    \end{center}%
  \end{center}%
}%


%-----------------------------------------------------------------------------------

\renewenvironment{abstract}%
  {\small\vspace{0.5mm}%
   \list{}{\rightmargin 2em%
           \leftmargin 2em}%
    \item{}{\bf Abstract}\hspace*{0.5em}\relax}%
   {\endlist}


%-----------------------------------------------------------------------------------

\newenvironment{keyword}%
  {\small%
    \list{}{\rightmargin 2em%
           \leftmargin 2em}%
                \item{}{\bf Key~words}\hspace*{0.5em}\relax }%
       {\endlist%
        }%

\newenvironment{pacs}%
  {\small%
    \list{}{\rightmargin 2em%
           \leftmargin 2em}%
                \item{}{\bf PACS}\hspace*{0.5em}\relax }%
       {\endlist%
        \vskip 6mm}%


%---------------------------------------------------------------

\newcommand{\acknowledgments}[1]{%
   {\it #1}%
  }


\makeatletter

%--------------------\section, \subsection--------------------------------------------------------------

\renewcommand \thesection {\bf\@arabic\c@section}  

\renewcommand\section{\@startsection {section}{1}{\z@}%
                                    {5mm \@plus.2ex \@minus .2ex}%
                                   {5mm \@plus.2ex \@minus .2ex}%
                                   {\normalfont\large\bfseries}}
\renewcommand\subsection{\@startsection{subsection}{2}{\z@}%
                                   %  {-2.25ex\@plus -1ex \@minus -.2ex}%
                                     {1.5ex \@plus .2ex}%
                                     {1.5ex \@plus .2ex}%
                                     {\normalfont\bfseries}}

\renewcommand\subsubsection{\renewcommand \thesection {\@arabic\c@section}
                            \@startsection{subsubsection}{3}{\z@}%
                                   %  {-2.25ex\@plus -1ex \@minus -.2ex}%
                                     {0.5ex}%
                                     {0.5ex}%
                                     {\normalfont}}
                                     
                                     
%----------------------------------------------------------------------------------------------

\renewcommand{\@biblabel}[1]{#1}
\renewcommand\refname{{\normalsize\bf References}}
\renewenvironment{thebibliography}[1]
     {\noindent\refname%
      \@mkboth{\MakeUppercase\refname}{\MakeUppercase\refname}%
      \footnotesize
      \list{\@biblabel{\@arabic\c@enumiv}}%
           {\settowidth\labelwidth{\@biblabel{#1}}%
            \leftmargin\labelwidth
            \advance\leftmargin\labelsep
            \@openbib@code
            \usecounter{enumiv}%
            \let\p@enumiv\@empty
            \renewcommand\theenumiv{\@arabic\c@enumiv}}%
      %\sloppy
      %\setlength{\itemsep}{-1.5mm}
      \setlength{\itemsep}{0mm}
      \setlength{\labelsep}{0.8em}
      \setlength{\parsep}{0mm}
      \setlength{\parskip}{0mm}
      \setlength{\topsep}{0mm}
      \setlength{\partopsep}{0mm}
      \clubpenalty4000
      \@clubpenalty \clubpenalty
      \widowpenalty4000%
      \sfcode`\.\@m}
     {\def\@noitemerr
       {\@latex@warning{Empty `thebibliography' environment}}%
      \endlist}

%---------------------------------------------------------------------------------

\newenvironment{mylabc}
                {%
                 \small
                 \let\\\@centercr
                 \list{}{\itemsep      \z@
                         \itemindent   -1em%
                         \listparindent0em
                         \leftmargin   3em
                         \rightmargin  2em}
                         \item\relax}
                {\endlist}


\makeatother




\fancypagestyle{myfoot}
{%
\fancyhf{}
\fancyhead[l]{\hspace{0.5em}\footnotesize CPC(HEP \& NP), 2009, {\bf 33}(X): \thepage---\pageref{LastPage}}
\fancyhead[r]{\footnotesize Vol.\;33, No.\;X,~ Xxx,\;2009\hspace{0.5em}}
\fancyhead[c]{\qquad\large\bf Chinese Physics C }
\fancyfoot[l]{\footnotesize\hspace{3mm}\raisebox{0.3ex}{$\scriptsize\copyright$}2009\! 
Chinese Physical Society and the Institute of High
Energy Physics of the Chinese\! Academy of Sciences and the Institute
of Modern Physics of the Chinese Academy of Sciences and IOP Publishing Ltd}
\renewcommand{\headrule}{\vskip 2pt
\hrule height0.4pt width\headwidth \vskip1pt
\hrule height0.4pt width\headwidth \vskip-1.8pt}
}%
\thispagestyle{myfoot}
 
\pagestyle{fancy}
\fancyhead{}
\fancyhead[lo]{\footnotesize \hspace{0.5em}No.\;X\hspace{0.5em}}
\fancyhead[ro,le]{\footnotesize \hspace{0.5em}\thepage\hspace{0.5em}}
\fancyhead[ce]{\footnotesize Chinese Physics C (HEP \& NP)}
\fancyhead[re]{\footnotesize \hspace{0.5em}Vol.\;33\hspace{0.5em}}
\fancyfoot[ce,co]{}
\renewcommand{\headrule}{\vskip 2pt  \hrule height0.4pt width\headwidth}

\makeatletter

\newcommand\figcaption{\def\@captype{figure}\caption}
\newcommand\tabcaption{\def\@captype{table}\caption}
\renewcommand\figurename{Fig.}

\long\def\@makecaption#1#2{%
\vskip\abovecaptionskip
\sbox\@tempboxa{#1.\quad #2}%
\ifdim \wd\@tempboxa >\hsize
  \begin{mylabc}
  \vspace{-2mm}
  {\small #1.\quad #2}%
  \vskip 1mm%
  \end{mylabc}\par
\else
   \global \@minipagefalse
   \hb@xt@\hsize{\hfil\box\@tempboxa\hfil}%
\fi
\vskip\belowcaptionskip}


\setcounter{page}{1}

\makeatother

%%
%% End of file `cpc-hepnp.cls'.

